Challenging local realism with human choices

A Bell test is a randomized trial that compares experimental observations against the philosophical worldview of local realism. A Bell test requires spatially distributed entanglement, fast and high-efficiency detection and unpredictable measurement settings. Although technology can satisfy the first two of these requirements, the use of physical devices to choose settings in a Bell test involves making assumptions about the physics that one aims to test. Bell himself noted this weakness in using physical setting choices and argued that human `free will' could be used rigorously to ensure unpredictability in Bell tests. Here we report a set of local-realism tests using human choices, which avoids assumptions about predictability in physics. We recruited about 100,000 human participants to play an online video game that incentivizes fast, sustained input of unpredictable selections and illustrates Bell-test methodology. The participants generated 97,347,490 binary choices, which were directed via a scalable web platform to 12 laboratories on five continents, where 13 experiments tested local realism using photons, single atoms, atomic ensembles, and superconducting devices. Over a 12-hour period on 30 November 2016, participants worldwide provided a sustained data flow of over 1,000 bits per second to the experiments, which used different human-generated data to choose each measurement setting. The observed correlations strongly contradict local realism and other realistic positions in bipartite and tripartite scenarios. Project outcomes include closing the `freedom-of-choice loophole' (the possibility that the setting choices are influenced by `hidden variables' to correlate with the particle properties), the utilization of video-game methods for rapid collection of human generated randomness, and the use of networking techniques for global participation in experimental science.

==> Authors.tex <==

\newcommand{\ICFOAddress}{ICFO-Institut de Ciencies Fotoniques, The Barcelona Institute of Science and Technology, 08860 Castelldefels (Barcelona), Spain} 
\newcommand{\ICREAAddress}{ICREA -- Instituci\'{o} Catalana de Re{c}erca i Estudis Avan\c{c}ats, 08010 Barcelona, Spain} 
\newcommand{\IQOQIAddress}{Institute for Quantum Optics and Quantum Information (IQOQI), Austrian Academy of Sciences, Boltzmanngasse 3, 1090 Vienna, Austria}
\newcommand{\UdeCAddress}{Departamento de F\'{i}sica, Universidad de Concepci\'{o}n, 160-C Concepci\'{o}n, Chile}
\newcommand{\CEFOPAddress}{Center for Optics and Photonics, Universidad de Concepci\'{o}n, Casilla 4016, Concepci\'{o}n, Chile}
\newcommand{\MSIAddress}{MSI-Nucleus for Advanced Optics, Universidad de Concepci\'{o}n, 160-C Concepci\'{o}n, Chile}
\newcommand{\CEFOPMSIAddress}{Center for Optics and Photonics and MSI-Nucleus for Advanced Optics, Universidad de Concepci\'{o}n, Casilla 4016, Concepci\'{o}n, Chile}
\newcommand{\DIEAddress}{Departamento de Ingenier\'{i}a El\'{e}ctrica, Universidad de Concepci\'{o}n,160-C Concepci\'{o}n, Chile}
\newcommand{\SevillaAddress}{Departamento de F\'{i}sica Aplicada II, Universidad de Sevilla, 41012 Sevilla, Spain}
\newcommand{\LinkopingAddress}{Department of Electrical Engineering, Link\"{o}ping University,  581 83 Link\"{o}ping, Sweden}
%\newcommand{\SapienzaAddress}{Dipartimento di Fisica, La Sapienza Universit\`{a} di Roma, I-00185 Roma, Italy}
\newcommand{\SapienzaAddress}{Dipartimento di Fisica, Sapienza Universit\`{a} di Roma, I-00185 Roma, Italy}
\newcommand{\EQUSAddress}{Centre for Engineered Quantum Systems, Centre for Quantum Computation and Communication Technology, School of Mathematics and Physics, University of Queensland, Brisbane, Queensland 4072, Australia}
\newcommand{\GriffithAddress}{Griffith University, Brisbane, Queensland 4111, Australia}
\newcommand{\CQDAddress}{Centre for Quantum Dynamics, Griffith University, Brisbane, Queensland 4111, Australia}
\newcommand{\CQCCTAddress}{Centre for Quantum Computation and Communication Technology, Griffith University, Brisbane, Queensland 4111, Australia}
\newcommand{\INFINIAddress}{Laboratoire de Physique de la Matire Condens\'{e}e, Universit\'{e} Nice Sophia Antipolis, CNRS UMR 7336, Parc Valrose, 06108 Nice Cedex 2, France}
\newcommand{\INPHYNIAddress}{Universit\'{e} C\^{o}te d'Azur, CNRS UMR 7010, Institut de Physique de Nice (INPHYNI), Parc Valrose, 06108 Nice Cedex 2, France}
\newcommand{\ETHQDLAddress}{Quantum Device Lab, Department of Physics, ETH Zurich, CH-8093 Zurich, Switzerland}
\newcommand{\ETHAddress}{Department of Physics, ETH Zurich, CH-8093 Zurich, Switzerland}
\newcommand{\LMUAddress}{Ludwig-Maximilians-Universit\"{a}t, 80799 M\"{u}nchen, Germany}
\newcommand{\MPQAddress}{Max-Planck-Institut f\"{u}r Quantenoptik, Hans-Kopfermann-Strasse 1, Garching 85748, Germany}
\newcommand{\UBAAddress}{Departamento de F\'{i}sica, FCEyN, UBA and IFIBA, Conicet, Pabell\'{o}n 1, Ciudad Universitaria, 1428 Buenos Aires, Argentina}

\newcommand{\DdCUBAAddress}{Departamento de Computaci\'{o}n, FCEyN, UBA and ICC, CONICET, Pabell\'{o}n 1, Ciudad Universitaria, 1428 Buenos Aires, Argentina}

\newcommand{\CITEDEFAddress}{DEILAP, CITEDEF \& CONICET, J.B. de La Salle 4397, 1603 Villa Martelli, Buenos Aires, Argentina}
\newcommand{\NISTAddress}{National Institute of Standards and Technology, 325 Broadway, Boulder, CO 80305, USA}
\newcommand{\IIPURFNAddress}{International Institute of Physics, Federal University of Rio Grande do Norte, 59070-405 Natal, Brazil}
\newcommand{\CENSEAddress}{CAS Center for Excellence in Superconducting Electronics, Shanghai 200050, China}
%\newcommand{\SIMITAddress}{Shanghai Institute of Microsystem and Information Technology, Chinese Academy of Sciences, Shanghai 200050, China}
\newcommand{\SIMITAddress}{State Key Laboratory of Functional Materials for Informatics, Shanghai Institute of Microsystem and Information Technology, Chinese Academy of Sciences, Shanghai 200050, China}
\newcommand{\PMOAddress}{Purple Mountain Observatory and Key Laboratory of Radio Astronomy, Chinese Academy of Sciences, 2 West Beijing Road, Nanjing 210008, China}
\newcommand{\TsinghuaAddress}{Center for Quantum Information, Institute for Interdisciplinary Information Sciences, Tsinghua University, Beijing 100084, China}
\newcommand{\USTCAddress}{Shanghai Branch, National Laboratory for Physical Sciences at Microscale and Dept. of Modern Physics, University of Science and Technology of China, Shanghai 230026, China}
\newcommand{\CASAddress}{Shanghai Branch, CAS Center for Excellence and Synergetic Innovation Center in Quantum Information and Quantum Physics, University of Science and Technology of China, Shanghai 230026, China}
\newcommand{\NUDTAddress}{School of Computer, NUDT, 410073 Changsha, China}

\newcommand{\BBTAuthorCoord}[1]{\BBTAuthor{#1} \affiliation{\ICFOAddress}}
%\renewcommand{\BBTAuthorCoord}[1]{}

\BBTAuthor{$^\dagger$The BIG Bell Test Collaboration: C. Abell\'{a}n}%agreed
\affiliation{\ICFOAddress}

\BBTAuthor{A. Ac\'{i}n}%agreed
%\email[]{}
\affiliation{\ICFOAddress}
\affiliation{\ICREAAddress}

\BBTAuthor{A. Alarc\'{o}n}%agreed
%\email[]{}
\affiliation{\CEFOPMSIAddress}
\affiliation{\DIEAddress}

\BBTAuthor{O. Alibart}
%\email[]{}
\affiliation{\INPHYNIAddress}

%\BBTAuthor{M. Almeida}
%%\email[]{}
%\affiliation{\EQUSAddress}

\BBTAuthor{C. K. Andersen}%agreed
%\email[]{chanders@phys.ethz.ch}
\affiliation{\ETHQDLAddress}

\BBTAuthor{F. Andreoli}%agreed
%\email[]{fra.andreoli@hotmail.it}
\affiliation{\SapienzaAddress}

\BBTAuthor{A. Beckert} %agreed
%\email[]{adbecker@phys.ethz.ch}
\affiliation{\ETHQDLAddress}

\BBTAuthorCoord{F. A. Beduini}


\BBTAuthor{A. Bendersky}%agreed
%\email[]{}
\affiliation{\DdCUBAAddress}

\BBTAuthor{M. Bentivegna}%agreed
%\email[]{marco.bentivegna@uniroma1.it}
\affiliation{\SapienzaAddress}

\BBTAuthor{P. Bierhorst}%agreed
%\email[]{}
\affiliation{\NISTAddress}

\BBTAuthor{D. Burchardt}%agreed
%\email[]{}
\affiliation{\LMUAddress}

\BBTAuthor{A. Cabello}%agreed
%\email[]{adan@us.es}
\affiliation{\SevillaAddress}

\BBTAuthor{J. Cari\~{n}e}%agreed
%\email[]{}
\affiliation{\CEFOPMSIAddress}
\affiliation{\DIEAddress}
\affiliation{\UdeCAddress}

\BBTAuthorCoord{S. Carrasco}%agreed
%\affiliation{\ICFOAddress}

\BBTAuthor{G. Carvacho}%agreed
%\email[]{gonzalocarvacho1@gmail.com}
\affiliation{\SapienzaAddress}

\BBTAuthor{D. Cavalcanti}%agreed
%\email[]{daniel.cavalcanti@icfo.es}
\affiliation{\ICFOAddress}


\BBTAuthor{R. Chaves}%agreed
%\email[]{rchaves@iip.ufrn.br}
\affiliation{\IIPURFNAddress}

\BBTAuthor{J. Cort\'{e}s-Vega}%agreed
%\email[]{}
\affiliation{\CEFOPMSIAddress}
\affiliation{\UdeCAddress}

\BBTAuthor{A. Cuevas}%agreed
%\email[]{alvaro.phys@gmail.com}
\affiliation{\SapienzaAddress}


\BBTAuthor{A. Delgado}%agreed
%\email[]{}
\affiliation{\CEFOPMSIAddress}
\affiliation{\UdeCAddress}

\BBTAuthor{H. de Riedmatten}%agreed
%\email[]{hugues.deriedmatten@icfo.es}
\affiliation{\ICFOAddress}
\affiliation{\ICREAAddress}

\BBTAuthor{C. Eichler}%agreed
%\email[]{christopher.eichler@phys.ethz.ch}
\affiliation{\ETHQDLAddress}

\BBTAuthor{P. Farrera}%agreed
%\email[]{Pau.Farrera@icfo.es}
\affiliation{\ICFOAddress}

%\BBTAuthor{M. Figueroa}
%%\email[]{}
%\affiliation{\DIEAddress}
%\affiliation{\MSIAddress}
%\affiliation{\CEFOPAddress}

\BBTAuthor{J. Fuenzalida}%agreed
%\email[]{jfuenzalida@udec.cl}
\affiliation{\CEFOPMSIAddress}
\affiliation{\UdeCAddress}
\affiliation{\IQOQIAddress}

\BBTAuthorCoord{M. Garc\'{i}a-Matos}


\BBTAuthor{R. Garthoff}%agreed
%\email[]{}
\affiliation{\LMUAddress}

\BBTAuthor{S. Gasparinetti}%agreed
%\email[]{simone.gasparinetti@phys.ethz.ch}
\affiliation{\ETHQDLAddress}

\BBTAuthor{T. Gerrits}%agreed
%\email[]{}
\affiliation{\NISTAddress}

\BBTAuthor{F. Ghafari Jouneghani}%agreed
%\email[]{farzad.ghafari@griffithuni.edu.au}
%\affiliation{\CQCCTAddress}
\affiliation{\CQCCTAddress}
\affiliation{\CQDAddress }

%\BBTAuthor{G. Gillett}
%%\email[]{}
%\affiliation{\EQUSAddress}

\BBTAuthor{S. Glancy}%agreed
%\email[]{}
\affiliation{\NISTAddress}

\BBTAuthor{E. S. G\'{o}mez}%agreed
%\email[]{}
\affiliation{\CEFOPMSIAddress}
\affiliation{\UdeCAddress}

\BBTAuthor{P. Gonz\'{a}lez}%agreed
%\email[]{estesepulveda@gmail.com}
\affiliation{\CEFOPMSIAddress}
\affiliation{\UdeCAddress}

\BBTAuthor{J.-Y. Guan}%agreed
%\email[]{}
\affiliation{\USTCAddress}
\affiliation{\CASAddress}

\BBTAuthor{J. Handsteiner}%agreed
%\email[]{johannes.handsteiner@univie.ac.at}
\affiliation{\IQOQIAddress}

\BBTAuthor{J. Heinsoo}
%\email[]{jheinsoo@phys..ch}
\affiliation{\ETHQDLAddress}

\BBTAuthor{G. Heinze}%agreed
%\email[]{Georg.Heinze@icfo.es}
\affiliation{\ICFOAddress}

\BBTAuthorCoord{A. Hirschmann}


\BBTAuthor{O. Jim\'{e}nez}%agreed
%\email[]{osvaldo.jimenez@icfo.eu}
\affiliation{\ICFOAddress}

\BBTAuthor{F. Kaiser}%agreed
%\email[]{Florian.KAISER@unice.fr}
\affiliation{\INPHYNIAddress}

\BBTAuthor{E. Knill}%agreed
%\email[]{}
\affiliation{\NISTAddress}
% 17 June 2017 by e-mail
%
%Dear Morgan,
%
%That "typeform" makes my browser choke (to many external scripts from
%randomly named cloud servers that have to be allowed). Here's the
%information you need.
%
%I agree to be a coauthor and have no corrections with respect to
%author information. I suppose I don't have to subscribe to the main
%conclusion, though it improved with Scott's input.  Your list of
%journals doesn't make sense to me, I think you'll figure out something
%though. In any case, it looks like you already formatted with a
%specific one in mind.
%
%Manny

\BBTAuthor{L. T. Knoll}%agreed
%\email[]{}
\affiliation{\CITEDEFAddress}
\affiliation{\UBAAddress}

\BBTAuthor{S. Krinner}
%\email[]{skrinner@phys.ethz.ch}
\affiliation{\ETHQDLAddress}

\BBTAuthor{P. Kurpiers}%agreed
%\email[]{kurphili@ethz.ch}
\affiliation{\ETHQDLAddress}

\BBTAuthor{M. A. Larotonda}%agreed
%\email[]{mlaroton@gmail.com}
\affiliation{\CITEDEFAddress}
\affiliation{\UBAAddress}

\BBTAuthor{J.-\AA. Larsson}%agreed
%\email[]{jan-ake.larsson@liu.se}
\affiliation{\LinkopingAddress}

\BBTAuthor{A. Lenhard}%agreed
%\email[]{Andreas.Lenhard@icfo.es}
\affiliation{\ICFOAddress}

\BBTAuthor{H. Li}%agreed
%\email[]{kshalm@gmail.com}
\affiliation{\SIMITAddress}
\affiliation{\CENSEAddress}


\BBTAuthor{M.-H. Li}%agreed
%\email[]{lmh0922@mail.ustc.edu.cn}
\affiliation{\USTCAddress}
\affiliation{\CASAddress}

\BBTAuthor{G. Lima}%agreed
%\email[]{}
\affiliation{\CEFOPMSIAddress}
\affiliation{\UdeCAddress}

\BBTAuthor{B. Liu}%agreed
%\email[]{liub90@unet.univie.ac.at}
\affiliation{\NUDTAddress}
\affiliation{\IQOQIAddress}

\BBTAuthor{Y. Liu}%agreed
%\email[]{yangphys@ustc.edu.cn}
\affiliation{\USTCAddress}
\affiliation{\CASAddress}

\BBTAuthor{I. H. L\'{o}pez Grande}%agreed
%\email[]{}
\affiliation{\CITEDEFAddress}
\affiliation{\UBAAddress}

\BBTAuthor{T. Lunghi}%agreed
%\email[]{Tommaso.LUNGHI@unice.fr}
\affiliation{\INPHYNIAddress}

\BBTAuthor{X. Ma}%agreed
%\email[]{}
\affiliation{\TsinghuaAddress}

\BBTAuthor{O. S. Maga\~{n}a-Loaiza}%agreed
%\email[]{}
\affiliation{\NISTAddress}

\BBTAuthor{P. Magnard}%agreed
%\email[]{paul.magnard@phys.ethz.ch}
\affiliation{\ETHQDLAddress}

\BBTAuthor{A. Magnoni}%agreed
%\email[]{}
\affiliation{\UBAAddress}

\BBTAuthorCoord{M. Mart\'{i}-Prieto}


\BBTAuthor{D. Mart\'{i}nez}%agreed
%\email[]{danielmartinezarias@gmail.com}
\affiliation{\CEFOPMSIAddress}
\affiliation{\UdeCAddress}

\BBTAuthor{ P. Mataloni}%agreed
%\email[]{paolo.mataloni@uniroma1.it}
\affiliation{\SapienzaAddress}

\BBTAuthor{A. Mattar}%agreed
%\email[]{ Alejandro.Mattar@icfo.eu}
\affiliation{\ICFOAddress}

\BBTAuthor{M. Mazzera}%agreed
%\email[]{Margherita.Mazzera@icfo.eu}
\affiliation{\ICFOAddress}

\BBTAuthor{R. P. Mirin}%agreed
%\email[]{}
\affiliation{\NISTAddress}

\BBTAuthor{M. W. Mitchell}%agreed
\email{morgan.mitchell@icfo.eu}
\affiliation{\ICFOAddress}
\affiliation{\ICREAAddress}

\BBTAuthor{S. Nam}%agreed	
%\email[]{}
\affiliation{\NISTAddress}

\BBTAuthor{M. Oppliger}
%\email[]{markus.oppliger@phys.ethz.ch}
\affiliation{\ETHQDLAddress}

%\BBTAuthor{N. Ortegel}
%%\email[]{}
%\affiliation{\LMUAddress}

\BBTAuthor{J.-W. Pan}%agreed
%\email[]{}
\affiliation{\USTCAddress}
\affiliation{\CASAddress}

\BBTAuthor{R. B. Patel}%agreed
%\email[]{r.patel@griffith.edu.au}
%\affiliation{\CQCCTAddress}
\affiliation{\CQCCTAddress}
\affiliation{\CQDAddress }

%\BBTAuthor{V. Pruneri}%agreed
%%\email[]{}
%\affiliation{\ICFOAddress}
%\affiliation{\ICREAAddress}

%MIME-Version: 1.0
%Received: from am5pr0901cu001.internal.outlook.com (2a01:111:e400:51cf::17) by
% DB5PR06MB1111.eurprd06.prod.outlook.com with HTTP via
% DB6PR07CA0098.EURPRD07.PROD.OUTLOOK.COM; Sun, 24 Sep 2017 06:07:49 +0000
%Received: from AM5PR0602MB2836.eurprd06.prod.outlook.com
% ([fe80::bc0f:7b4c:c846:24f3]) by AM5PR0602MB2836.eurprd06.prod.outlook.com
% ([fe80::bc0f:7b4c:c846:24f3%18]) with mapi id 15.20.0077.011; Sun, 24 Sep
% 2017 06:07:48 +0000
%From: Valerio Pruneri <Valerio.Pruneri@icfo.eu>
%To: Morgan Mitchell <morgan.mitchell@icfo.eu>
%Subject: Re: Title of talk
%Thread-Topic: Title of talk
%Thread-Index: AQHTM+7r6XfKH37Se0mr0QOUiME8nqLBgaJWgAINZWQ=
%Date: Sun, 24 Sep 2017 08:07:48 +0200
%Message-ID:
%	<AM5PR0602MB2836A1E59251F2F9A0782E56E4650@AM5PR0602MB2836.eurprd06.prod.outlook.com>
%References:
%	<AM5PR0602MB2836BB44BA89B2E99ACD5F67E4670@AM5PR0602MB2836.eurprd06.prod.outlook.com>,<DB5PR06MB11114300BDABBC70380A081DEF670@DB5PR06MB1111.eurprd06.prod.outlook.com>
%In-Reply-To:
%	<DB5PR06MB11114300BDABBC70380A081DEF670@DB5PR06MB1111.eurprd06.prod.outlook.com>
%Accept-Language: en-GB, en-US
%Content-Language: en-US
%X-MS-Exchange-Organization-AuthAs: Internal
%X-MS-Exchange-Organization-AuthMechanism: 04
%X-MS-Exchange-Organization-AuthSource:
%	AM5PR0602MB2836.eurprd06.prod.outlook.com
%X-MS-Has-Attach:
%X-MS-Exchange-Organization-Network-Message-Id:
%	d412a0ed-7294-43ea-1350-08d50312952b
%X-MS-Exchange-Organization-SCL: -1
%X-MS-TNEF-Correlator:
%X-MS-Exchange-Organization-RecordReviewCfmType: 0
%x-ms-publictraffictype: Email
%X-Microsoft-Exchange-Diagnostics:
%	1;DB5PR06MB1111;27:Ix8g3OAk7pN+LdDSTVGoalN2b76+31kDki7mP0738m6gddICzfRNWAAv+doPrWnv1vsyDYhoLZJ1TuSqaepvAdvmIAo9zupaRKu4ypE+j1dE1dMTxniiY2VfftiyZO6m
%Content-Type: text/html; charset="us-ascii"
%
%<html>
%<head>
%<meta http-equiv="Content-Type" content="text/html; charset=us-ascii">
%<meta content="text/html; charset=us-ascii">
%<meta content="text/html; charset=us-ascii">
%</head>
%<body>
%<div dir="auto" style="direction:ltr; margin:0; padding:0; font-family:sans-serif; font-size:11pt; color:black; background-color:white">
%Please remove my name from the human Bell test paper.<br>
%<br>
%</div>
%<div dir="auto" style="direction:ltr; margin:0; padding:0; font-family:sans-serif; font-size:11pt; color:black; background-color:white">
%<div dir="auto" style="direction:ltr; margin:0; padding:0; font-family:sans-serif; font-size:11pt; color:black; background-color:white">
%Get <a href="https://aka.ms/ghei36">Outlook for Android</a></div>
%<br>
%</div>
%<hr tabindex="-1" style="display:inline-block; width:98%">
%<div id="divRplyFwdMsg" dir="ltr"><font face="Calibri, sans-serif" color="#000000" style="font-size:11pt"><b>From:</b> Morgan Mitchell<br>
%<b>Sent:</b> Saturday, September 23, 2017 12:47:21 AM<br>
%<b>To:</b> Valerio Pruneri<br>
%<b>Subject:</b> Re: Title of talk</font>
%<div>&nbsp;</div>
%</div>
%<div>
%<div dir="auto" style="direction:ltr; margin:0; padding:0; font-family:sans-serif; font-size:11pt; color:black; background-color:white">
%what title did u see?&nbsp; They gave it the chip title. I talked about methodology and the title was metrological approach... and I gave you ( and your people and valencia but mostly you) credit for the integration.&nbsp;&nbsp;
%<br>
%<br>
%</div>
%<div dir="auto" style="direction:ltr; margin:0; padding:0; font-family:sans-serif; font-size:11pt; color:black; background-color:white">
%<div dir="auto" style="direction:ltr; margin:0; padding:0; font-family:sans-serif; font-size:11pt; color:black; background-color:white">
%Get <a href="https://aka.ms/ghei36">Outlook for Android</a></div>
%<br>
%</div>
%<hr tabindex="-1" style="display:inline-block; width:98%">
%<div id="divRplyFwdMsg" dir="ltr"><font face="Calibri, sans-serif" color="#000000" style="font-size:11pt"><b>From:</b> Valerio Pruneri<br>
%<b>Sent:</b> Saturday, September 23, 2017 12:05:36 AM<br>
%<b>To:</b> Morgan Mitchell<br>
%<b>Subject:</b> Title of talk</font>
%<div>&nbsp;</div>
%</div>
%<div>
%<div dir="auto" style="direction:ltr; margin:0; padding:0; font-family:sans-serif; font-size:11pt; color:black; background-color:white">
%Morgan<br>
%</div>
%<div dir="auto" style="direction:ltr; margin:0; padding:0; font-family:sans-serif; font-size:11pt; color:black; background-color:white">
%I was surprised to see the title of your talk at qcrypt and not being aware of it.<br>
%</div>
%<div dir="auto" style="direction:ltr; margin:0; padding:0; font-family:sans-serif; font-size:11pt; color:black; background-color:white">
%Valerio<br>
%<br>
%</div>
%<div dir="auto" style="direction:ltr; margin:0; padding:0; font-family:sans-serif; font-size:11pt; color:black; background-color:white">
%<div dir="auto" style="direction:ltr; margin:0; padding:0; font-family:sans-serif; font-size:11pt; color:black; background-color:white">
%Get <a href="https://aka.ms/ghei36">Outlook for Android</a></div>
%<br>
%</div>
%</div>
%</div>
%</body>
%</html>


\BBTAuthor{G. J. Pryde}%agreed
%\email[]{geoff.pryde@gmail.com}
%\affiliation{\CQCCTAddress}
\affiliation{\CQCCTAddress}
\affiliation{\CQDAddress }

\BBTAuthor{D. Rauch}%agreed
%\email[]{dominik.rauch@univie.ac.at}
\affiliation{\IQOQIAddress}

\BBTAuthor{K. Redeker}%agreed
%\email[]{}
\affiliation{\LMUAddress}

\BBTAuthor{D. Riel\"{a}nder}%agreed
%\email[]{daniel.rielaender@gmx.de}
\affiliation{\ICFOAddress}


\BBTAuthor{M. Ringbauer}%agreed
\affiliation{\EQUSAddress}
%\email[]{m.ringbauer@uq.edu.au}

\BBTAuthor{T. Roberson}
%\email[]{}
\affiliation{\EQUSAddress}

\BBTAuthor{W. Rosenfeld}%agreed
%\email[]{Wenjamin.Rosenfeld@physik.uni-muenchen.de}
\affiliation{\LMUAddress}

\BBTAuthor{Y. Salath\'{e}}%agreed
%\email[]{ysalathe@phys.ethz.ch}
\affiliation{\ETHQDLAddress}

\BBTAuthor{L. Santodonato}%agreed
%\email[]{santodonato.luca@hotmail.it}
\affiliation{\SapienzaAddress}

\BBTAuthor{G. Sauder}%agreed
%\email[]{Gregory.SAUDER@unice.fr}
\affiliation{\INPHYNIAddress}

\BBTAuthor{T. Scheidl}%agreed
%\email[]{thomas.scheidl@univie.ac.at}
\affiliation{\IQOQIAddress}

\BBTAuthor{C. T. Schmiegelow}%agreed
%\email[]{schmiegelow@df.uba.ar} % need to check but I think itÕs this one
\affiliation{\UBAAddress}

\BBTAuthor{F. Sciarrino}%agreed
%\email[]{fabio.sciarrino@uniroma1.it}
\affiliation{\SapienzaAddress}

\BBTAuthor{A. Seri}%agreed
%\email[]{Alessandro.Seri@icfo.eu}
\affiliation{\ICFOAddress}

% NIST Node
\BBTAuthor{L. K. Shalm}%agreed
%\email[]{kshalm@gmail.com}
\affiliation{\NISTAddress}

\BBTAuthor{S.-C. Shi}%agreed
%\email[]{kshalm@gmail.com}
\affiliation{\PMOAddress}




\BBTAuthor{S. Slussarenko}%agreed
%\email[]{s.slussarenko@griffith.edu.au}
%\affiliation{\CQCCTAddress}
\affiliation{\CQCCTAddress}
\affiliation{\CQDAddress }

\BBTAuthor{M. J. Stevens}%agreed
%\email[]{}
\affiliation{\NISTAddress}


\BBTAuthor{S. Tanzilli}
%\email[]{Sebastien.TANZILLI@unice.fr}
\affiliation{\INPHYNIAddress}

%\BBTAuthor{N. Tischler}
%%\email[]{n.tischler@griffith.edu.au}
%\affiliation{\CQCCTAddress}
%\affiliation{\GriffithAddress}

\BBTAuthor{F. Toledo}%agreed
%\email[]{}
\affiliation{\CEFOPMSIAddress}
\affiliation{\UdeCAddress}

\BBTAuthor{J. Tura }%agreed
%\email[]{}
\affiliation{\ICFOAddress}
\affiliation{\MPQAddress}

%IQOQI authors
\BBTAuthor{R. Ursin}%agreed
%\email[]{rupert.ursin@oeaw.ac.at}
\affiliation{\IQOQIAddress}

\BBTAuthor{P. Vergyris}%agreed
%\email[]{Panagiotis.VERGYRIS@unice.fr}
\affiliation{\INPHYNIAddress}

\BBTAuthor{V. B. Verma}
\affiliation{\NISTAddress}

\BBTAuthor{T. Walter}
%\email[]{thwalter@phys.ethz.ch}
\affiliation{\ETHQDLAddress}

\BBTAuthor{A. Wallraff}%agreed
%\email[]{andreas.wallraff@phys.ethz.ch}
\affiliation{\ETHQDLAddress}

\BBTAuthor{Z. Wang}%agreed
%\email[]{}
\affiliation{\SIMITAddress}
\affiliation{\CENSEAddress}

\BBTAuthor{H. Weinfurter}%agreed
%\email[]{harald.weinfurter@physik.uni-muenchen.de}
\affiliation{\LMUAddress}
\affiliation{\MPQAddress }%%As seen as an affilitation in other papers

\BBTAuthor{M. M. Weston}%agreed
\affiliation{\CQCCTAddress}
\affiliation{\CQDAddress }

%\BBTAuthor{T. Weinhold}
%%\email[]{}
%\affiliation{\EQUSAddress}

\BBTAuthor{A. G. White}%agreed
%\email[]{agx.white@gmail.com}
\affiliation{\EQUSAddress}

\BBTAuthor{C. Wu}%agreed
%\email[]{}
\affiliation{\USTCAddress}
\affiliation{\CASAddress}

\BBTAuthor{G. B. Xavier}%agreed
\affiliation{\CEFOPMSIAddress}
\affiliation{\DIEAddress}
\affiliation{\LinkopingAddress}
%\email[]{gxavier@udec.cl}

\BBTAuthor{L. You}%agreed
%\email[]{}
\affiliation{\SIMITAddress}
\affiliation{\CENSEAddress}

\BBTAuthor{X. Yuan}%agreed
%\email[]{}
\affiliation{\TsinghuaAddress}



\BBTAuthor{A. Zeilinger}%agreed
%\email[]{zeilina6@univie.ac.at}
\affiliation{\IQOQIAddress}

\BBTAuthor{Q. Zhang}%agreed
%\email[]{qiangzh@ustc.edu.cn }
\affiliation{\USTCAddress}
\affiliation{\CASAddress}

\BBTAuthor{W. Zhang}%agreed
%\email[]{kshalm@gmail.com}
\affiliation{\SIMITAddress}
\affiliation{\CENSEAddress}


\BBTAuthor{J. Zhong}%agreed
%\email[]{jqzhong@pmo.ac.cn}
\affiliation{\PMOAddress}


%\BBTAuthor{OTHER BBT}% PI
%%\email[]{qiangzh@ustc.edu.cn }
%\affiliation{still need to add these}


%% ADDRESSES BY INSTITUTION
%
%\BBTAuthor{The BIG Bell Test collaboration: Carlos Abellan}
%\affiliation{\ICFOAddress}
%
%\BBTAuthor{Morgan W. Mitchell}
%\affiliation{\ICFOAddress}
%\affiliation{\ICREAAddress}
%
%
%%IQOQI authors
%\BBTAuthor{R. Ursin}
%%\email[]{rupert.ursin@oeaw.ac.at}
%\affiliation{\IQOQIAddress}
%\BBTAuthor{A. Zeilinger}
%%\email[]{zeilina6@univie.ac.at}
%\affiliation{\IQOQIAddress}
%\BBTAuthor{T. Scheidl}
%%\email[]{thomas.scheidl@univie.ac.at}
%\affiliation{\IQOQIAddress}
%
%%Universidad de Concepci—n Node authors
%\BBTAuthor{F. Toledo}
%%\email[]{}
%\affiliation{\UdeCAddress}
%\affiliation{\MSIAddress}
%\affiliation{\CEFOPAddress}
%
%\BBTAuthor{P. Gonzalez}
%%\email[]{}
%\affiliation{\UdeCAddress}
%\affiliation{\MSIAddress}
%\affiliation{\CEFOPAddress}
%
%\BBTAuthor{J. Cort\'{e}s}
%%\email[]{}
%\affiliation{\UdeCAddress}
%\affiliation{\MSIAddress}
%\affiliation{\CEFOPAddress}
%
%\BBTAuthor{A. Delgado}
%%\email[]{}
%\affiliation{\UdeCAddress}
%\affiliation{\MSIAddress}
%\affiliation{\CEFOPAddress}
%
%\BBTAuthor{G. Lima}
%%\email[]{}
%\affiliation{\UdeCAddress}
%\affiliation{\MSIAddress}
%\affiliation{\CEFOPAddress}
%
%\BBTAuthor{A. Alarc\'{o}n}
%%\email[]{}
%\affiliation{\DIEAddress}
%\affiliation{\MSIAddress}
%\affiliation{\CEFOPAddress}
%\BBTAuthor{J. Cari\~{n}e}
%%\email[]{}
%\affiliation{\DIEAddress}
%\affiliation{\MSIAddress}
%\affiliation{\CEFOPAddress}
%
%\BBTAuthor{M. Figueroa}
%%\email[]{}
%\affiliation{\DIEAddress}
%\affiliation{\MSIAddress}
%\affiliation{\CEFOPAddress}
%
%\BBTAuthor{A. Cabello}
%%\email[]{adan@us.es}
%\affiliation{\SevillaAddress}
%
%
%\BBTAuthor{ J. Larsson}
%%\email[]{jan-ake.larsson@liu.se}
%\affiliation{\LinkopingAddress}
%
%\BBTAuthor{ P. Mataloni}
%%\email[]{paolo.mataloni@uniroma1.it}
%\affiliation{\SapienzaAddress}
%
%\BBTAuthor{A. Cuevas}
%%\email[]{alvaro.phys@gmail.com}
%\affiliation{\SapienzaAddress}
%
%\BBTAuthor{G. Carvacho}
%%\email[]{gonzalocarvacho1@gmail.com}
%\affiliation{\SapienzaAddress}
%
%\BBTAuthor{F. Sciarrino}
%%\email[]{fabio.sciarrino@uniroma1.it}
%\affiliation{\SapienzaAddress}
%
%\BBTAuthor{G. B. Xavier}
%\affiliation{\DIEAddress}
%\affiliation{\MSIAddress}
%\affiliation{\CEFOPAddress}
%%\email[]{gxavier@udec.cl}
%
%%EQUS Queensland node
%\BBTAuthor{M. Almeida}
%%\email[]{}
%\affiliation{\EQUSAddress}
%
%\BBTAuthor{G. Gillett}
%%\email[]{}
%\affiliation{\EQUSAddress}
%
%\BBTAuthor{J. Romero}
%%\email[]{}
%\affiliation{\EQUSAddress}
%
%\BBTAuthor{M. Ringbauer}
%\affiliation{\EQUSAddress}
%%\email[]{m.ringbauer@uq.edu.au}
%
%\BBTAuthor{T. Weinhold}
%%\email[]{}
%\affiliation{\EQUSAddress}
%
%\BBTAuthor{A. White}
%%\email[]{agx.white@gmail.com}
%\affiliation{\EQUSAddress}
%
%% Griffith University Node
%\BBTAuthor{R. Patel}
%%\email[]{r.patel@griffith.edu.au}
%\affiliation{\CQCCTAddress}
%\affiliation{\GriffithAddress}
%
%\BBTAuthor{S. Slussarenko}
%%\email[]{s.slussarenko@griffith.edu.au}
%\affiliation{\CQCCTAddress}
%\affiliation{\GriffithAddress}
%
%\BBTAuthor{N. Tischler}
%%\email[]{n.tischler@griffith.edu.au}
%\affiliation{\CQCCTAddress}
%\affiliation{\GriffithAddress}
%
%\BBTAuthor{G. Pryde}
%%\email[]{geoff.pryde@gmail.com}
%\affiliation{\CQCCTAddress}
%\affiliation{\GriffithAddress}
%
%%USTC Node
%\BBTAuthor{Y. Liu}
%%\email[]{yangphys@ustc.edu.cn}
%\affiliation{\USTCAddress}
%\affiliation{\CASAddress}
%
%\BBTAuthor{C. Wu}
%%\email[]{}
%\affiliation{\USTCAddress}
%\affiliation{\CASAddress}
%
%\BBTAuthor{J. Guang}
%%\email[]{}
%\affiliation{\USTCAddress}
%\affiliation{\CASAddress}
%
%\BBTAuthor{X. Ma}
%%\email[]{}
%\affiliation{\TsinghuaAddress}
%
%\BBTAuthor{X. Yuan}
%%\email[]{}
%\affiliation{\TsinghuaAddress}
%
%\BBTAuthor{L. You}
%%\email[]{}
%\affiliation{\SIMITAddress}
%
%
%\BBTAuthor{Z. Wang}
%%\email[]{}
%\affiliation{\SIMITAddress}
%
%\BBTAuthor{Q. Zhang}% PI
%%\email[]{qiangzh@ustc.edu.cn }
%\affiliation{\USTCAddress}
%\affiliation{\CASAddress}
%
%\BBTAuthor{J. Pan}%PI
%%\email[]{}
%\affiliation{\USTCAddress}
%\affiliation{\CASAddress}
%
%%Nice Node
%\BBTAuthor{F. Kaiser}
%%\email[]{Florian.KAISER@unice.fr}
%\affiliation{\INFINIAddress}
%
%\BBTAuthor{T. Lunghi}
%%\email[]{Tommaso.LUNGHI@unice.fr}
%\affiliation{\INFINIAddress}
%
%\BBTAuthor{G. Sauder}
%%\email[]{Gregory.SAUDER@unice.fr}
%\affiliation{\INFINIAddress}
%
%\BBTAuthor{P. Vergyris}
%%\email[]{Panagiotis.VERGYRIS@unice.fr}
%\affiliation{\INFINIAddress}
%
%\BBTAuthor{O. Alibart}
%%\email[]{}
%\affiliation{\INFINIAddress}
%
%\BBTAuthor{S. Tanzilli}
%%\email[]{Sebastien.TANZILLI@unice.fr}
%\affiliation{\INFINIAddress}
%
%%ICFO Node
%%Experiment 1
%
%\BBTAuthor{G.Heinze}
%%\email[]{Georg.Heinze@icfo.es}
%\affiliation{\ICFOAddress}
%
%\BBTAuthor{P. Farrera}
%%\email[]{Pau.Farrera@icfo.es}
%\affiliation{\ICFOAddress}
%
%
%%Experiment 2, no idea of the order of the names
%\BBTAuthor{A. Seri}
%%\email[]{Alessandro.Seri@icfo.eu}
%\affiliation{\ICFOAddress}
%
%\BBTAuthor{A. Lenhard}
%%\email[]{Andreas.Lenhard@icfo.es}
%\affiliation{\ICFOAddress}
%
%\BBTAuthor{M. Mazzera}
%%\email[]{Margherita.Mazzera@icfo.eu}
%\affiliation{\ICFOAddress}
%
%\BBTAuthor{H. de Riedmatten}%PI
%%\email[]{hugues.deriedmatten@icfo.es}
%\affiliation{\ICFOAddress}
%\affiliation{\ICREAAddress}
%
%%ETH Zurich
%\BBTAuthor{K. Andersen}
%%\email[]{}
%\affiliation{\ETHQDLAddress}
%
%\BBTAuthor{A. Beckert}
%%\email[]{}
%\affiliation{\ETHQDLAddress}
%
%\BBTAuthor{C. Eichler}
%%\email[]{}
%\affiliation{\ETHQDLAddress}
%
%\BBTAuthor{J. Heinsoo}
%%\email[]{jheinsoo@phys.ethz.ch}
%\affiliation{\ETHQDLAddress}
%
%\BBTAuthor{S. Krinner}
%%\email[]{}
%\affiliation{\ETHQDLAddress}
%
%\BBTAuthor{P. Kurpiers}
%%\email[]{kurphili@ethz.ch}
%\affiliation{\ETHQDLAddress}
%
%\BBTAuthor{P. Magnard}
%%\email[]{}
%\affiliation{\ETHQDLAddress}
%
%\BBTAuthor{M. Oppliger}
%%\email[]{}
%\affiliation{\ETHQDLAddress}
%
%\BBTAuthor{Y. Salath\'{e}}
%%\email[]{}
%\affiliation{\ETHQDLAddress}
%
%\BBTAuthor{T. Walter}
%%\email[]{}
%\affiliation{\ETHQDLAddress}
%
%\BBTAuthor{A. Wallraff}
%%\email[]{andreas.wallraff@phys.ethz.ch}
%\affiliation{\ETHQDLAddress}
%
%%LMU Munich Team
%\BBTAuthor{D. Burchardt}
%%\email[]{}
%\affiliation{\LMUAddress}
%\BBTAuthor{K. Redeker}
%%\email[]{}
%\affiliation{\LMUAddress}
%
%\BBTAuthor{R. Garthoff}
%%\email[]{}
%\affiliation{\LMUAddress}
%
%\BBTAuthor{N. Ortegel}
%%\email[]{}
%\affiliation{\LMUAddress}
%
%\BBTAuthor{W. Rosenfeld}%Project leader
%%\email[]{Wenjamin.Rosenfeld@physik.uni-muenchen.de}
%\affiliation{\LMUAddress}
%
%\BBTAuthor{H. Weinfurter}%PI
%%\email[]{harald.weinfurter@physik.uni-muenchen.de}
%\affiliation{\LMUAddress}
%\affiliation{\MPQAddress }%%As seen as an affilitation in other papers
%
%%CITEDEF Buenos Aires Node
%
%\BBTAuthor{L. T. Knoll}
%%\email[]{}
%\affiliation{\CITEDEFAddress}
%
%
%\BBTAuthor{I. H. L\'{o}pez Grande}
%%\email[]{}
%\affiliation{\CITEDEFAddress}
%
%\BBTAuthor{C. T. Schmiegelow}
%%\email[]{schmiegelow@df.uba.ar} % need to check but I think itÕs this one
%\affiliation{\UBAAddress}
%
%\BBTAuthor{A. Bendersky}
%%\email[]{}
%\affiliation{\UBAAddress}
%
%\BBTAuthor{A. Magnoni}
%%\email[]{}
%\affiliation{\UBAAddress}
%
%\BBTAuthor{M. A. Larotonda}
%%\email[]{mlaroton@gmail.com}
%\affiliation{\CITEDEFAddress}
%\affiliation{\UBAAddress}
%
%% NIST Node
%\BBTAuthor{K. Shalm}
%%\email[]{kshalm@gmail.com}
%\affiliation{\NISTAddress}
%
%\BBTAuthor{M. Stevens}
%%\email[]{}
%\affiliation{\NISTAddress}
%
%\BBTAuthor{S. W. Nam}
%%\email[]{}
%\affiliation{\NISTAddress}
%
%% Sapienza Node, careful, Fabio Sciarrino appears twice, he is PI of this experiment and collaborator in the Concepcion experiment
%\BBTAuthor{F. Andreoli}
%%\email[]{fra.andreoli@hotmail.it}
%\affiliation{\SapienzaAddress}
%
%\BBTAuthor{M. Bentivegna}
%%\email[]{marco.bentivegna@uniroma1.it}
%\affiliation{\SapienzaAddress}
%
%\BBTAuthor{G. Carvacho}
%%\email[]{gonzalocarvacho1@gmail.com}%% Please note this name appears twice!
%\affiliation{\SapienzaAddress}
%
%\BBTAuthor{L. Santodonato}
%%\email[]{santodonato.luca@hotmail.it}
%\affiliation{\SapienzaAddress}
%
%\BBTAuthor{R. Chaves}
%%\email[]{rchaves@iip.ufrn.br}
%\affiliation{\IIPURFNAddress}
%
%\BBTAuthor{F. Sciarrino}%% Please note this name appears twice!
%%\email[]{fabio.sciarrino@uniroma1.it}
%\affiliation{\SapienzaAddress}


%carlos.abellan@icfo.eu,
%antonio.acin@icfo.eu,
%g.pryde@griffith.edu.au,
%agx.white@gmail.com,
%yangphys@ustc.edu.cn,
%qiangzh@ustc.edu.cn,
%thomas.scheidl@univie.ac.at,
%rupert.ursin@oeaw.ac.at,
%zeilina6@univie.ac.at,
%paolo.mataloni@uniroma1.it,
%fabio.sciarrino@uniroma1.it,
%adan@us.es,
%jan-ake.larsson@liu.se,
%Wenjamin.Rosenfeld@physik.uni-muenchen.de,
%harald.weinfurter@physik.uni-muenchen.de,
%andreas.wallraff@phys.ethz.ch,
%Sebastien.TANZILLI@unice.fr,
%hugues.deriedmatten@icfo.es,
%mlaroton@gmail.com,
%gxavier@udec.cl,
%kshalm@gmail.com


==> BA.tex <==
%no .tex source here.  This is just to allow TexShop to invoke bibtex.

==> EQUS.tex <==
%no .tex source here.  This is just to allow TexShop to invoke bibtex.

==> ETHZ.tex <==
%no .tex source here.  This is just to allow TexShop to invoke bibtex.

==> GU.tex <==
%no .tex source here.  This is just to allow TexShop to invoke bibtex.

==> ICFOONE.tex <==
%no .tex source here.  This is just to allow TexShop to invoke bibtex.

==> ICFOTWO.tex <==
%no .tex source here.  This is just to allow TexShop to invoke bibtex.

==> IQOQI.tex <==
%no .tex source here.  This is just to allow TexShop to invoke bibtex.

==> LMU.tex <==
%no .tex source here.  This is just to allow TexShop to invoke bibtex.

==> NICE.tex <==
%no .tex source here.  This is just to allow TexShop to invoke bibtex.

==> NIST.tex <==
%no .tex source here.  This is just to allow TexShop to invoke bibtex.

==> ROMA.tex <==
%no .tex source here.  This is just to allow TexShop to invoke bibtex.

==> USTC.tex <==
%no .tex source here.  This is just to allow TexShop to invoke bibtex.

==> UdeC.tex <==
%no .tex source here.  This is just to allow TexShop to invoke bibtex.
